Efficient Adversarial Training without Attacking: Worst-Case-Aware Robust Reinforcement Learning

Recent studies reveal that a well-trained deep reinforcement learning (RL) policy can be particularly vulnerable to adversarial perturbations on input observations. Therefore, it is crucial to train RL agents that are robust against any attacks with a bounded budget. Existing robust training methods in deep RL either treat correlated steps separately, ignoring the robustness of long-term rewards, or train the agents and RL-based attacker together, doubling the computational burden and sample complexity of the training process. In this work, we propose a strong and efficient robust training framework for RL, named Worst-case-aware Robust RL (WocaR-RL) that directly estimates and optimizes the worst-case reward of a policy under bounded l_p attacks without requiring extra samples for learning an attacker. Experiments on multiple environments show that WocaR-RL achieves state-of-the-art performance under various strong attacks, and obtains significantly higher training efficiency than prior state-of-the-art robust training methods. The code of this work is available at https://github.com/umd-huang-lab/WocaR-RL.

==> checklist.tex <==
\section*{Checklist}
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See our abstract and Section~\ref{sec:intro}.}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss the limitations in Appendix~\ref{app:limit}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discuss the potential negative societal impacts in Appendix~\ref{app:limit}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Our paper conforms to the guidelines.}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Appendix~\ref{app:theory}.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix~\ref{app:theory}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{app:exp:imp}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{For each empirical result, we report error bars.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See efficiency analysis in Appendix~\ref{app:exp:eff}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> draft.tex <==




if we want to focus on the between clean value and worst case value 
after the introduction and prelim
- though not surprising, clean value and worst-case value are "competing objectives" 

clean prediction + attacked prediction
clean value + worst-case value

- existing methods for improving the robustness, 
- point out that the trade-off also exists for different states
- to balance the robustness of different states


1. 
2. compute the worst case value
3. algorithm efficiently improve both values
4. good performance

\section{1.Intro}
RL is vulnerable to adversarial perturbations.

I: value matters instead of individual points (why we have state weights) (the Pong example)

SA-DQN / RADIAL-DQN: do not consider the worst case value (consider individual states separately, similarly to supervised learning)

II: efficiency matters (why we propose the bellman operator)

Existing methods achieve good performance and robustness by doing xxx. Not efficient enough

inefficiency mainly due to the evaluating of the worst case value
ATLA(sa, pa): learn an RL attacker against the current policy which requires extra samples
Ours: use the past samples to directly estimate the worst case performance of the current policy

What we propose and contributions


\section{2.}
\input{related work}

\section{3.}
% \subsection{3.1 Motivation of the Algorithm}
% Competing objectives and different robustness across states
% Achieve both high value and high robustness, but they can be competing. we show the toy example where the best policy may get the worst value under attack.

% Theory example

\subsection{3.1 }
How to weight states

\subsection{3.2}
Worst case Bellman Operator

\section{4. Algorithm Description}


\section{5. }

\subsection{5.1}
main results

\subsection{5.2 discussion on the trade-off between two values}
Theory example and the empirical evidence

==> fig_curve_workshop.tex <==
\begin{figure}[t]
% \vspace{-0.5em}
    \centering
    \rotatebox{90}{\scriptsize{\qquad \quad Walker2d}}
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\fighome/curve_atla/walker_sa.tex}}
        \vspace{-1.5em}
        % \label{sfig:example_worst}
    \end{subfigure}
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\fighome/curve_atla/walker_pa.tex}}
        \vspace{-1.5em}
        % \label{sfig:example_worst}
    \end{subfigure}
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\fighome/curve_atla/walker_na.tex}}
        \vspace{-1.5em}
        % \label{sfig:example_worst}
    \end{subfigure}\\
    \rotatebox{90}{\scriptsize{\qquad \quad \ Hopper}}
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\fighome/curve_atla/hopper_sa.tex}}
        \vspace{-1.5em}
        % \label{sfig:example_worst}
    \end{subfigure}
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\fighome/curve_atla/hopper_pa.tex}}
        \vspace{-1.5em}
        % \label{sfig:example_worst}
    \end{subfigure}
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\fighome/curve_atla/hopper_na.tex}}
        % \includegraphics[width=1.12\columnwidth, trim={0 0 0 20},clip]{\fighome/trade-off/walker.pdf}
        \vspace{-1.5em}
        % \label{sfig:example_state}
    \end{subfigure}
    \vspace{-1em}
    \caption{\small{ \textbf{Robustness, Efficiency and High Natural Performance of WocaR-PPO.}
    \textbf{(Left two columns)} Learning curves
    % (mean $\pm$ standard deviation)
    of rewards under SA-RL and PA-AD \textit{(the strongest)} attacks during training. \textbf{(Rightmost column)} Average episode natural rewards v.s. average worst rewards under attacks. Each row shows the performance of baselines and \ourppo on one environment. Shaded regions are computed over 20 random seeds. Results under more attack radius $\epsilon$'s are in Appendix~\ref{app:exp:eps}.}}
    \label{fig:mujoco_workshop}
\vspace{-1em}
\end{figure}

==> fig_mujoco.tex <==
\begin{figure}[!t]
\vspace{-1em}
\centering
\hspace{-0.5em}\includegraphics[width=0.9\columnwidth, trim={20 0 20 30},clip]{\fighome/curve/walker.pdf}
\vspace{-1em}
\caption{Average episode rewards $\pm$ standard deviation over 50 episodes for robust agents against different attacks on Walker2d.}
\label{fig:mujoco}
\vspace{-1.5em}
\end{figure}

==> figures/curve_atla/legend.tex <==



==> figures/results/mujoco.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}[scale=0.6]

\definecolor{color0}{rgb}{0.917647058823529,0.917647058823529,0.949019607843137}
\definecolor{color1}{rgb}{0.556862745098039,0.729411764705882,0.258823529411765}
\definecolor{color2}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}
\definecolor{color3}{rgb}{0.596078431372549,0.556862745098039,0.835294117647059}
\definecolor{color4}{rgb}{0.984313725490196,0.756862745098039,0.368627450980392}
\definecolor{color5}{rgb}{0.886274509803922,0.290196078431373,0.2}

\begin{groupplot}[group style={group size=4 by 1}]
\nextgroupplot[
axis background/.style={fill=color0},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, fill=color0},
tick align=outside,
x grid style={white},
xlabel={Hopper},
xmajorgrids,
xmajorticks=false,
xmin=-0.211, xmax=2.561,
xtick style={color=white!15!black},
xtick={0.51,2.01},
xticklabels={Natural rewards, Worst rewards},
y grid style={white},
ymajorgrids,
ymajorticks=false,
ymin=0, ymax=4500,
ytick style={color=white!15!black}
]
\draw[draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}] (axis cs:-0.085,0) rectangle (axis cs:0.085,3167);
\addlegendimage{ybar,ybar legend,draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}}
\addlegendentry{Vanilla PPO}

\draw[draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}] (axis cs:1.415,0) rectangle (axis cs:1.585,160);
\draw[draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.085,0) rectangle (axis cs:0.255,3705);
\addlegendimage{ybar,ybar legend,draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}}
\addlegendentry{SA-PPO}

\draw[draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:1.585,0) rectangle (axis cs:1.755,856);
\draw[draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}] (axis cs:0.255,0) rectangle (axis cs:0.425,3291);
\addlegendimage{ybar,ybar legend,draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}}
\addlegendentry{ATLA-PPO}

\draw[draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}] (axis cs:1.755,0) rectangle (axis cs:1.925,1232);
\draw[draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.425,0) rectangle (axis cs:0.595,3449);
\addlegendimage{ybar,ybar legend,draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}}
\addlegendentry{PA-ATLA-PPO}

\draw[draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:1.925,0) rectangle (axis cs:2.095,2521);
\draw[draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.595,0) rectangle (axis cs:0.765,3687);
\addlegendimage{ybar,ybar legend,draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}}
\addlegendentry{RADIAL-PPO}

\draw[draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:2.095,0) rectangle (axis cs:2.265,1036);
\draw[draw=white,fill=color5,opacity=0.9,line width=0.32pt] (axis cs:0.765,0) rectangle (axis cs:0.935,3616);
\addlegendimage{ybar,ybar legend,draw=white,fill=color5,opacity=0.9,line width=0.32pt}
\addlegendentry{RQ-PPO(ours)}

\draw[draw=white,fill=color5,opacity=0.9,line width=0.32pt] (axis cs:2.265,0) rectangle (axis cs:2.435,2579);
\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0,2625)
--(axis cs:0,3709);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.5,24)
--(axis cs:1.5,296);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.17,3703)
--(axis cs:0.17,3707);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.67,835)
--(axis cs:1.67,877);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.34,2691)
--(axis cs:0.34,3891);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.84,882)
--(axis cs:1.84,1582);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.51,3212)
--(axis cs:0.51,3686);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.01,2196)
--(axis cs:2.01,2846);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.68,3607)
--(axis cs:0.68,3767);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.18,894)
--(axis cs:2.18,1178);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.85,3517)
--(axis cs:0.85,3715);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.35,2334)
--(axis cs:2.35,2824);



\nextgroupplot[
axis background/.style={fill=color0},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, fill=color0},
tick align=outside,
x grid style={white},
xlabel={Walker2d},
xmajorgrids,
xmajorticks=false,
xmin=-0.211, xmax=2.561,
xtick style={color=white!15!black},
xtick={0.425,1.925},
xticklabels={Natural rewards,Worst rewards},
y grid style={white},
ymajorgrids,
ymajorticks=false,
ymin=500, ymax=5000,
ytick style={color=white!15!black}
]
\draw[draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}] (axis cs:-0.085,0) rectangle (axis cs:0.085,4472);
\draw[draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}] (axis cs:1.415,0) rectangle (axis cs:1.585,804);
\draw[draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.085,0) rectangle (axis cs:0.255,4487);
\draw[draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:1.585,0) rectangle (axis cs:1.755,1042);
\draw[draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}] (axis cs:0.255,0) rectangle (axis cs:0.425,3842);
\draw[draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}] (axis cs:1.755,0) rectangle (axis cs:1.925,1224);
\draw[draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.425,0) rectangle (axis cs:0.595,4178);
\draw[draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:1.925,0) rectangle (axis cs:2.095,2248);
\draw[draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.595,0) rectangle (axis cs:0.765,2143);
\draw[draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:2.095,0) rectangle (axis cs:2.265,674);
\draw[draw=white,fill=color5,opacity=0.9,line width=0.32pt] (axis cs:0.765,0) rectangle (axis cs:0.935,4076);
\draw[draw=white,fill=color5,opacity=0.9,line width=0.32pt] (axis cs:2.265,0) rectangle (axis cs:2.435,2722);
\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0,4137)
--(axis cs:0,4807);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.5,674)
--(axis cs:1.5,934);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.17,4426)
--(axis cs:0.17,4548);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.67,689)
--(axis cs:1.67,1395);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.34,3367)
--(axis cs:0.34,4317);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.84,454)
--(axis cs:1.84,1994);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.51,3649)
--(axis cs:0.51,4707);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.01,2117)
--(axis cs:2.01,2379);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.68,1990)
--(axis cs:0.68,2296);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.18,580)
--(axis cs:2.18,768);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.85,3581)
--(axis cs:0.85,4571);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.35,2370)
--(axis cs:2.35,3074);


\nextgroupplot[
axis background/.style={fill=color0},
axis line style={white},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, fill=color0},
tick align=outside,
x grid style={white},
xlabel={Halfcheetah},
xmajorgrids,
xmajorticks=false,
xmin=-0.211, xmax=2.561,
xtick style={color=white!15!black},
xtick={0.425,1.925},
xticklabels={Natural rewards,Worst rewards},
y grid style={white},
ymajorgrids,
ymajorticks=false,
ymin=-1000, ymax=8000,
ytick style={color=white!15!black}
]
\draw[draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}] (axis cs:-0.085,0) rectangle (axis cs:0.085,7117);
\draw[draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}] (axis cs:1.415,0) rectangle (axis cs:1.585,-356);
\draw[draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.085,0) rectangle (axis cs:0.255,3632);
\draw[draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:1.585,0) rectangle (axis cs:1.755,2512);
\draw[draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}] (axis cs:0.255,0) rectangle (axis cs:0.425,6157);
\draw[draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}] (axis cs:1.755,0) rectangle (axis cs:1.925,2576);
\draw[draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.425,0) rectangle (axis cs:0.595,6289);
\draw[draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:1.925,0) rectangle (axis cs:2.095,3840);
\draw[draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.595,0) rectangle (axis cs:0.765,4735);
\draw[draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:2.095,0) rectangle (axis cs:2.265,2743);
\draw[draw=white,fill=color5,opacity=0.9,line width=0.32pt] (axis cs:0.765,0) rectangle (axis cs:0.935,5503);
\draw[draw=white,fill=color5,opacity=0.9,line width=0.32pt] (axis cs:2.265,0) rectangle (axis cs:2.435,4258);
\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0,7019)
--(axis cs:0,7215);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.5,-763)
--(axis cs:1.5,51);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.17,3612)
--(axis cs:0.17,3652);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.67,2496)
--(axis cs:1.67,2528);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.34,5305)
--(axis cs:0.34,7009);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.84,2028)
--(axis cs:1.84,3124);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.51,5947)
--(axis cs:0.51,6631);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.01,3567)
--(axis cs:2.01,4113);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.68,4703)
--(axis cs:0.68,4767);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.18,2625)
--(axis cs:2.18,2861);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.85,5445)
--(axis cs:0.85,5561);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.35,4086)
--(axis cs:2.35,4430);


\nextgroupplot[
axis background/.style={fill=color0},
axis line style={white},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black,
  fill=color0
},
tick align=outside,
x grid style={white},
xlabel={Ant},
xmajorgrids,
xmajorticks=false,
xmin=-0.211, xmax=2.561,
xtick style={color=white!15!black},
xtick={0.425,1.925},
xticklabels={Natural rewards,Worst rewards},
y grid style={white},
ymajorgrids,
ymajorticks=false,
ymin=-3000, ymax=7000,
ytick style={color=white!15!black}
]
\draw[draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}] (axis cs:-0.085,0) rectangle (axis cs:0.085,5687);
\draw[draw=white,fill=color1,opacity=0.75,line width=0.32pt,postaction={pattern=crosshatch, pattern color=white, fill opacity=0.75}] (axis cs:1.415,0) rectangle (axis cs:1.585,-2580);
\draw[draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.085,0) rectangle (axis cs:0.255,4292);
\draw[draw=white,fill=color2,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:1.585,0) rectangle (axis cs:1.755,-1296);
\draw[draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}] (axis cs:0.255,0) rectangle (axis cs:0.425,5359);
\draw[draw=white,fill=color3,opacity=0.75,line width=0.32pt,postaction={pattern=north west lines, pattern color=white, fill opacity=0.75}] (axis cs:1.755,0) rectangle (axis cs:1.925,220);
\draw[draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.425,0) rectangle (axis cs:0.595,5469);
\draw[draw=white,fill=white!46.6666666666667!black,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:1.925,0) rectangle (axis cs:2.095,2986);
\draw[draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:0.595,0) rectangle (axis cs:0.765,5087);
\draw[draw=white,fill=color4,opacity=0.75,line width=0.32pt,postaction={pattern=north east lines, pattern color=white, fill opacity=0.75}] (axis cs:2.095,0) rectangle (axis cs:2.265,1568);
\draw[draw=white,fill=color5,opacity=0.9,line width=0.32pt] (axis cs:0.765,0) rectangle (axis cs:0.935,5196);
\draw[draw=white,fill=color5,opacity=0.9,line width=0.32pt] (axis cs:2.265,0) rectangle (axis cs:2.435,3097);
\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0,4929)
--(axis cs:0,6445);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.5,-3452)
--(axis cs:1.5,-1708);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.17,3908)
--(axis cs:0.17,4676);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.67,-2219)
--(axis cs:1.67,-373);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.34,5206)
--(axis cs:0.34,5512);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:1.84,-118)
--(axis cs:1.84,558);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.51,5363)
--(axis cs:0.51,5575);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.01,2622)
--(axis cs:2.01,3350);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.68,4952)
--(axis cs:0.68,5222);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.18,1324)
--(axis cs:2.18,1812);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:0.85,4671)
--(axis cs:0.85,5721);

\path [draw=white!41.1764705882353!black, line width=0.52pt]
(axis cs:2.35,2868)
--(axis cs:2.35,3326);


\end{groupplot}

\end{tikzpicture}


==> figures/trade-off/cartpole.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.917647058823529,0.917647058823529,0.949019607843137}
\definecolor{color1}{rgb}{0.301960784313725,0.686274509803922,0.290196078431373}

\begin{axis}[
axis background/.style={fill=color0},
axis line style={white},
tick align=outside,
x grid style={white},
xlabel={Scores (Performance)},
xmajorgrids,
xmajorticks=false,
xmin=100, xmax=200,
xtick style={color=white!15!black},
y grid style={white},
ylabel={Worst-case Scores (Robustness)},
ymajorgrids,
ymajorticks=false,
ymin=20, ymax=110,
ytick style={color=white!15!black}
]
\addplot [draw=color1, fill=color1, mark=*, only marks, opacity=0.4]
table{%
x  y
184.67128241919 49.3397605262513
191.353158005388 45.9820700414061
182.634442341196 30.7253722698485
183.690559743289 41.5157484276786
183.241088695786 35.0801404143877
184.847672723241 35.6170228267049
192.527765436145 31.9211618172724
183.691207870439 36.3320999003201
183.543830634145 44.3326405392814
187.063567322968 44.2250630932398
186.031169967056 48.7090876028804
183.671420861061 39.0715946217248
184.536890726025 34.0973821997674
193.70844294583 34.6411815571113
181.189929857398 32.3530635962004
190.437760126042 44.6299096313743
180.157259442108 37.3674094837327
192.408450557018 38.215290865932
185.040821856374 49.1457837855046
186.533920415996 49.7587541836154
188.586785065378 43.1035176238658
192.756819920581 31.4410787759723
186.724403822935 34.6914921989833
186.898211527999 32.6631559125012
192.967120467831 45.6170492780746
184.592758751615 35.7929347799067
191.401048421554 41.9900341640316
189.568449010992 37.02365653208
188.011914235618 45.7009828874765
188.461232478316 35.5986396844885
168.986684914716 59.6214734718782
165.870960673818 59.4225907686291
168.289943549341 40.1529907416079
158.52469980954 48.707950985871
176.298553006826 58.5473046112667
174.194169996824 55.9622420725557
175.24304395225 40.0213900136871
174.172808578314 50.6690031492261
168.738282846846 48.4683287316644
161.893859881662 48.4619604812225
159.684235087893 43.7150210990618
161.254758675186 55.9898294327202
164.198323086779 55.3258377707734
174.88716010145 56.8026278481083
161.805272440395 57.3386428150443
175.566579829624 58.0393517682039
165.731656711672 56.4511483381197
167.863230014891 42.4443967391803
161.500841447613 53.0171851040202
163.455136420333 58.9156017223565
167.547910635671 44.1833320377153
170.188062641443 42.2234141253231
172.851768816256 56.3316517955269
162.086509816497 57.9519658458381
174.515930755936 55.4877843193019
175.40172382598 53.4905907606273
171.144251719398 42.4201536642539
167.289938950762 57.7882480011992
170.12790305803 48.4646227514507
174.073236662052 59.1584745714537
158.39522950192 60.2296532668644
142.262473620791 59.6357978294376
161.516617989071 57.3706441280574
129.766936009395 58.8392493606135
128.448361985075 53.3025299767493
125.031577199973 54.0596641784712
143.793952048846 57.36564577591
148.024227925723 55.5567822212527
147.237982363609 54.3744751133717
161.129777119699 55.7489947762261
129.554963260526 54.7348371011069
137.419665282546 53.5121240803417
131.745566160524 60.8525594391978
130.064900928407 53.7133332494089
150.191999776018 58.8712505778967
135.743620490571 61.8485975129166
128.361202740422 60.2769524312539
159.267131871783 56.9665744696555
149.344020874934 59.50987490024
147.880579955811 61.5377066658165
112.415397620293 88.9360117973271
110.522427690849 92.4744514664438
110.896755648811 87.7158841764626
125.726710840978 88.9119362939824
121.363436936063 84.1509877019803
104.840578223589 86.1202494155325
121.014416599462 79.7140668532058
133.090562273492 88.0756431450169
118.898060344337 91.9632941290982
119.729196401511 93.504945625884
123.286067869064 84.6420865600629
133.387965320691 96.4653309512186
118.587512534695 81.0818586028546
113.241558916682 91.7892042394283
123.622473310338 87.7835135415186
132.991281638008 74.6364003243909
127.079422205631 88.3003257970356
132.850599514018 85.2641880553585
120.752814614173 83.816032366634
131.022766333961 75.6726336119328
119.85753493317 78.7329653099375
117.47306344867 93.0967265944684
117.633610318917 94.9793850315914
117.69345417109 85.2799748864533
119.44056134605 77.4265803992912
115.601802189774 83.7599002504243
118.222245394014 93.4894636574385
119.662807346084 80.2021244546286
115.223323245961 89.1868883644667
118.388265987668 81.046448533485
115.958313332017 89.4755748361046
116.843103596741 84.4588494978675
118.36370494134 86.750444231078
116.355736274703 88.6176006699869
115.620015056104 80.9003571839362
119.275314833902 79.6680220220618
119.978904159446 86.3152963816516
119.064611201268 83.4853644245687
118.416715002913 77.7438861935846
116.243799734663 77.3948674150964
};
\end{axis}

\end{tikzpicture}


==> table_mujoco_full.tex <==
\begin{table*}[!t]
\vspace{-0.5em}
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{0.9\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
% \setlength{\arrayrulewidth}{1pt}
\begin{tabular}{p{2.7cm}<{\centering}| p{2cm}<{\centering} | p{2cm}<{\centering} | p{2cm}<{\centering} | p{2cm}<{\centering} | p{2cm}<{\centering} | p{2cm}<{\centering} | p{2cm}<{\centering} | p{2cm}<{\centering}}
\toprule
\multirow{3}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Hopper} } & \multicolumn{2}{c|}{\textbf{Walker2d} } & 
\multicolumn{2}{c|}{\textbf{Halfcheetah}} &
\multicolumn{2}{c}{\textbf{Ant}} \\
\cline{2-9}
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Natural}\\\textbf{Reward}\end{tabular}} & \textbf{PA-AD} & 
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Natural}\\\textbf{Reward}\end{tabular}} & \textbf{PA-AD} &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Natural}\\\textbf{Reward}\end{tabular}} & \textbf{PA-AD} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Natural}\\\textbf{Reward}\end{tabular}} & \textbf{PA-AD}\\
 & & $\epsilon$= 0.075 & & $\epsilon$= 0.05 & & $\epsilon$= 0.15 & & $\epsilon$= 0.15\\
\hline
PPO (vanilla) & 3167 $\pm$ 542 & 160 $\pm$ 136 & 4472 $\pm$ 635 & 804 $\pm$ 130 & \textbf{7117 $\pm$ 98} & -356 $\pm$ 407 & \textbf{5687 $\pm$ 758} & -2580 $\pm$ 872 \\
SA-PPO & \textbf{3705 $\pm$ 2} & 856 $\pm$ 21 & \textbf{4487 $\pm$ 61} & 1042 $\pm$ 353  & 3632 $\pm$ 20 & 2512 $\pm$ 16 & 4292 $\pm$ 384 & -1296 $\pm$ 923\\
ATLA-PPO & 3291 $\pm$ 600 & 1232 $\pm$ 350 & 3842 $\pm$ 475  & 1224 $\pm$ 770  &  6157 $\pm$ 852 & 2576 $\pm$ 548 & 5359 $\pm$ 153 & 220 $\pm$ 338 \\
PA-ATLA-PPO & 3449 $\pm$ 237 & 2521 $\pm$ 325 & 4178 $\pm$ 529  & 2248 $\pm$ 131  & 6289 $\pm$ 342 & 3840 $\pm$ 273 & 5469 $\pm$ 106 & 2986 $\pm$ 364 \\
RADIAL-PPO & 3687 $\pm$ 80 & 1036 $\pm$ 142 & 2143 $\pm$ 153  & 674 $\pm$ 94  &  4683 $\pm$ 97 & 2074 $\pm$ 168 & 4376 $\pm$ 254 & 1549 $\pm$ 304\\
\cellcolor{lightgray}{\textbf{\ourppo (Ours)}} & \cellcolor{lightgray}{3616 $\pm$ 99} & \cellcolor{lightgray}{\textbf{2579 $\pm$ 245}} & \cellcolor{lightgray}{4076 $\pm$ 495}  & \cellcolor{lightgray}{\textbf{2722 $\pm$ 352}}   & \cellcolor{lightgray}{5872 $\pm$ 68} & \cellcolor{lightgray}{\textbf{4258 $\pm$ 172}} & \cellcolor{lightgray}{5596 $\pm$ 525} & \cellcolor{lightgray}{\textbf{3097 $\pm$ 229}} \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Average episode rewards $\pm$ standard deviation over 50 episodes on five baselines and \ourppo on four MuJoCo environments. Natural reward and rewards under PA-AD attacks are reported. Under each column corresponding to an evaluation metric, we bold the best results. And the row for the most robust agent is highlighted as \colorbox{lightgray}{gray}.}
\label{tab:mujoco}
\vspace{-1em}
\end{table*}


